Probabilistic Algorithm for Polynomial Optimization over a Real Algebraic Set

Let $f, f_1, \ldots, f_\nV$ be polynomials with rational coefficients in the indeterminates $\bfX=X_1, \ldots, X_n$ of maximum degree $D$ and $V$ be the set of common complex solutions of $\F=(f_1,\ldots, f_\nV)$. We give an algorithm which, up to some regularity assumptions on $\F$, computes an exact representation of the global infimum $f^\star=\inf_{x\in V\cap\R^n} f\Par{x}$, i.e. a univariate polynomial vanishing at $f^\star$ and an isolating interval for $f^\star$. Furthermore, this algorithm decides whether $f^\star$ is reached and if so, it returns $x^\star\in V\cap\R^n$ such that $f\Par{x^\star}=f^\star$. This algorithm is probabilistic. It makes use of the notion of polar varieties. Its complexity is essentially cubic in $\Par{\nV D}^n$ and linear in the complexity of evaluating the input. This fits within the best known deterministic complexity class $D^{O(n)}$. We report on some practical experiments of a first implementation that is available as a Maple package. It appears that it can tackle global optimization problems that were unreachable by previous exact algorithms and can manage instances that are hard to solve with purely numeric techniques. As far as we know, even under the extra genericity assumptions on the input, it is the first probabilistic algorithm that combines practical efficiency with good control of complexity for this problem.

==> complexity.tex <==
\section{Complexity analysis}\label{sec:complexity}
\subsection{Geometric degree bounds}\label{sec:degbounds}
In this section, we assume that the polynomial $f$ and the polynomials
$f_i$ have degree $\leq D$.  Recall that the degree of an irreducible
algebraic variety $V\subset\C^n$ is defined as the maximum finite
cardinal of $V\cap L$ for every linear subspace $L\subset\C^n$. If $V$
is not irreducible, $\deg V $ is defined as the sum of the degrees of
its irreducible components. The degree of a hypersurface $\Variety{f}$
is bounded by $\deg f$. Given a variety $V=\Variety{g_1,\dots,g_p}$,
we denote by $\delta\Par{V}$ the maximum of the degrees
$\deg\Par{V\Par{g_1,\dots,g_i}}$, for $1\leq i\leq p$.  Our goal in
this section is to estimate the degree of the geometric objects
computed in the algorithm. Obtaining such estimations is relevant
since the complexity of the algorithm relies on these degrees.


\begin{proposition}\label{prop:degbounds}
  For all $\bfA\in\GLnQ\cap\NEZOS$, for $1\leq i\leq d$,
  $\delta\Par{\VVA{f^\bfA}{\F^\bfA}{i}}$ and
  $\delta\Par{\VPC{f^\bfA}{\F^\bfA}{i}}$ are bounded by
$D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$.
\end{proposition}
\begin{proof}
  Let $E_1=\Variety{f^\bfA-T, \F^\bfA}$ and denote by $E_2,E_3,\dots,
  E_p$ the zero-sets of each minor of size $n-d+1$ of
  $\jac{\left[f^\bfA,\F^\bfA\right]}{i+1}$. Then for $2\leq j\leq p$,
  each $E_j$ has degree bounded by $\Par{n-d+1}\Par{D-1}$. Moreover,
  it is straightforward to see that $E_1$ has degree bounded by
  $D^{n-d}$ and dimension $d$. Let $1\leq k\leq p$. Then using
  \cite[Proposition 2.3]{HeSc80} we get
  \begin{equation}
    \deg\Par{\bigcap_{1\leq j\leq k} E_j}\leq\deg E_1\Par{\max_{1<j\leq k}\deg E_j}^{\dim E_1}. \label{eq:HeSc}
  \end{equation}

  In particular,
  \[\deg\Par{\bigcap_{1\leq j\leq k} E_j}\leq D^{n-d}\Par{\Par{n-d+1}\Par{D-1}}^{d}.\]
  By B\'ezout's inequality (\cite[Proposition 2.3]{HeSc80}), it
  follows that the degree of $\displaystyle\bigcap_{1\leq j\leq k} E_j\cap
  \Variety{\bfX_{\leq i-1}}$ is also bounded by
  $D^{n-d}\Par{\Par{n-d+1}\Par{D-1}}^{d}$. Finally, this implies that
  \begin{equation}
    \delta\Par{\VVA{f^\bfA}{\F^\bfA}{i}}\leq
    D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d}.\label{eq:geomdegbound}
  \end{equation}

  It remains to prove that $\delta\Par{\VPC{f^\bfA}{\F^\bfA}{i}}\leq
  D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$. From the
  above inequality \eqref{eq:geomdegbound}, we deduce that
  \[\delta\Par{\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus{\critfVbfA}}}\leq
  D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d}.\]

  Finally, we apply \cite[Proposition 2.3]{HeSc80} with the varieties
  $F_1,\dots,F_t$, where
  \[F_1=
  \ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus{\critfVbfA}}\] and
  $F_2,F_3,\dots,F_t$ are the zero-sets of each minor defining
  $\critfVbfA$.  Since these minors have degree bounded by
  $\Par{n-d+1}\Par{D-1}$, this quantity bounds the degree of the
  hypersurfaces they define. By Proposition \ref{prop:finite}, $F_1 =
  \ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\critfVbfA}$ has
  dimension $1$. Then inequality \eqref{eq:HeSc} becomes
  \[\deg\Par{\bigcap_{1\leq j\leq t} F_j}\leq
  D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d}\times \Par{n-d+1}\Par{D-1}.\] We conclude  that
  \[\delta\Par{\VPC{f^\bfA}{\F^\bfA}{i}}\leq
  D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}.\]
\end{proof}


\subsection{Complexity estimates}
Let $\bfA\in\GLnQ\cap\NEZOS$. Let
$\mathbf{F}=\left\{f_1,\dots,f_\nV\right\}\subset\PolRing$, $f$ and
$g$ in $\PolRing$ of degree bounded by $D$ that are given by a
straight-line program (SLP) of size $\leq L$. Recall that $d$ denotes
the dimension of $V=\Variety{\mathbf{F}}$.

To estimate the complexity of our algorithm, we use the the geometric
resolution algorithm \cite{GiLeSa01, lecerf2003} and its
subroutines. This is a probabilistic algorithm for polynomial system
solving. In the sequel, a geometric resolution is a representation of
a variety by a parametrization. A lifting fiber is a data from which a
geometric resolution can be recovered. We refer to
\cite{GiLeSa01,lecerf2003, schost03} for precise statements.

We describe the geometric resolution probabilistic subroutines and
their complexity used to represent the varieties in our algorithm in
Section \ref{sec:geomressubroutines}. The complexity depends on the
geometric degree and the maximal size of the SLPs representing the
polynomials involved in the definition of our varieties. Then Section
\ref{sec:sizeSLP} is devoted to give bounds on the size of these
SLPs. Then estimations of the complexity of our subroutines and the
main algorithm are given in the rest of this Section.


\subsubsection{Geometric Resolution subroutines}\label{sec:geomressubroutines}
\begin{itemize}
\item \textsf{GeometricSolveRRS} \cite[Section 7]{GiLeSa01}: let
  $\F=\left\{f_1,\dots,f_n\right\}$ and $g$ be polynomials in
  $\Q[\mathbf{X}]$ of degree $\leq D$ and given by a straight-line
  program of length $E$. Assume that $\F$ defines a {\em reduced
    regular sequence} in the open subset $\left\{g\neq
    0\right\}$. This routine returns a geometric resolution of
  $\ZariskiClosure{\Variety{\mathbf{F}}\setminus \Variety{g}}$ in
  probabilistic time
  \[\widetilde{O}\Par{\Par{nE+n^4}\Par{D\delta\Par{\Variety{\F}}}^2}.\]
\item \textsf{GeometricSolve} \cite[Section 5.2]{lecerf2003}: let
  $\mathbf{F}$ and $g$ be as above of degree $\leq D$ given by a straight-line program of
  length $E$. This routine returns an equidimensional decomposition of
  $\ZariskiClosure{\Variety{\mathbf{F}}\setminus \Variety{g}}$,
  encoded by a set of irreducible lifting fibers in probabilistic time
  \[\widetilde{O}\Par{sn^4\Par{nE+n^4}\Par{D\delta\Par{\Variety{\F}}}^3}.\]
\item \textsf{SplitFiber} \cite[Section 3.4]{lecerf2003}: given a
  lifting fiber $F$ of a variety $\Variety{\F}$, it returns a set of
  irreducible lifting fibers of $\Variety{\F}$ in time 
  \[\widetilde{O}\Par{sn^4\Par{nE+n^4}\Par{D\delta\Par{\Variety{\F}}}^3}.\]
\item \textsf{LiftCurve} \cite[Section 3.3]{lecerf2003}: given an irreducible
  lifting fiber $F$ of the above output,  this
  routine returns a rational parametrization of the lifted curve of
  $F$ in time
  \[\widetilde{O}\Par{sn^4\Par{nE+n^4}\Par{D\delta\Par{\Variety{\F}}}^2}.\]
\item \textsf{OneDimensionalIntersect} \cite[Section 6]{GiLeSa01}: let
  $\F$ be as above such that $\IdealAngle{\F}$ is a $1$-dimensional ideal,
  $\mathfrak{I}$ be a geometric resolution of $\IdealAngle{\F}$, and
  $f$ and $g$ be polynomials. In case of success, the routine returns
  a rational parametrization of
  $\ZariskiClosure{\Variety{\mathfrak{I}+f}\cap\Variety{g}}$ in time
  \[\widetilde{O}\Par{n\Par{E+n^2}\Par{D\delta\Par{\Variety{\F}}^2}}.\]
\item \textsf{LiftParameter} \cite[Section 4.2]{schost03}: let $T$ be
  a parameter and let $\mathcal{P}_T$ be a set of polynomials in
  $\Q(T)[X_1,\dots,X_n]$ be given by a straight-line program of length
  $E$. Let $t\in\R$ be a generic point and $\mathcal{P}_t$ be the
  polynomial system specialized at $t$. If $\Variety{\mathcal{P}_t}$
  is $0$-dimensional, the routine takes as input a geometric
  resolution of $\mathcal{P}_t$ and returns a parametric geometric
  resolution of $\mathcal{P}_t$ in time
  \[\widetilde{O}\Par{\Par{nE+n^4+n}\delta\Par{\Variety{\mathcal{P}_t}}
    \Par{4\delta\Par{\Variety{\mathcal{P}_T}}+1}}.\]
\item \textsf{Difference} \cite[Section 4.1]{lecerf2003}: let $V_1$,
  $V_2$ be algebraic varieties defined as the vanishing set of
  polynomial families given by a straight line program of length $E$
  and represented by lifting fibers. In case of success, the routine
  returns a fiber $F$ of the components of
  $\ZariskiClosure{V_1\setminus V_2}$ in time
  \[\widetilde{O}\Par{n^4\Par{nE+n^4}\delta\Par{V_2}^2\delta\Par{V_1}}.\]
\end{itemize}


\subsubsection{Size of SLP}\label{sec:sizeSLP}
We want to estimate some parameters depending on the inputs of the
geometric resolution routines, that are the polynomials defining the
varieties $\VVA{f^\bfA}{\F^\bfA}{i}$ and
$\VPC{f^\bfA}{\F^\bfA}{i}$. Since bounds on
$\delta\Par{\VVA{f^\bfA}{\F^\bfA}{i}}$ and
$\delta\Par{\VPC{f^\bfA}{\F^\bfA}{i}}$ have been obtained in the
previous section, it remains to estimates the size of the
straight-line programs representing these polynomials. These
polynomials are either a polynomial $f^\bfA$ or $f^\bfA_i$ or a minor
of size $n-d+1$ of the Jacobian matrix
$\jac{\left[f^\bfA,\F^\bfA\right]}{i+1}$. The polynomials $f$ and
$f_i$ are given as a SLP of size $L$. Then $f^\bfA$ and $f^\bfA_i$,
can be represented by a SLP of size $O\left(L + n^2\right)$. Then we
estimate the size of the minors. Let $\omega$ be the
matrix-multiplication exponent.

\begin{proposition}
  Each minors of size $n-d+1$ of
  $\jac{\left[f^\bfA,\F^\bfA\right]}{i+1}$ can be represented by a SLP
  of size
  $\widetilde{O}\left(\left(n-d+1\right)^{\omega/2+2}\left(L+n^2\right)\right)$.
\end{proposition}
\begin{proof}
  The partial derivatives appearing in the Jacobian matrix come from
  $f^\bfA$ and $f^\bfA_i$, represented by a SLP of size
  $O\left(L+n^2\right)$. According to \cite{BaurStrassen}, each
  partial derivative $\frac{\partial f^\bfA_i}{\partial x_j}$ and
  $\frac{\partial f^\bfA}{\partial x_j}$ can be represented by a SLP
  of size $O\left(L+n^2\right)$. Moreover, according to \cite{Ka92},
  the determinant of an $n\times n$ matrix can be computed using only
  $+$, $-$ and $\times$ in
  $\widetilde{O}\left(\left(n-d+1\right)^{\omega/2+2}\right)$
  operations. We combine these two results to conclude the proof.
\end{proof}

\begin{remark}
  Recall that $\omega\leq 3$. In the sequel, to lighten the
  expressions of complexity, we replace the above complexity
  $\widetilde{O}\left(\left(n-d+1\right)^{\omega/2+2}\left(L+n^2\right)\right)$
  with $\widetilde{O}\left(n^{4}\left(L+n^2\right)\right)$, that is
  less accurate but that dominates the first one.
\end{remark}


\subsubsection{Computation of  $\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$}\label{sec:complexVVA}
Recall that the algebraic variety $\VVA{f^\bfA}{F^\bfA}{i}$ is defined as the vanishing set
of
\begin{itemize}
\item the polynomials $f^\bfA_1, \ldots, f^\bfA_\nV$,
\item the minors of size $n-d+1$ of $\jacc{\left[f^\bfA,\F^\bfA\right], i+1}$,
\item and the variables $X_1, \ldots, X_{i-1}$.
\end{itemize}

The algebraic set $\VVA{f^\bfA}{F^\bfA}{i}$ can be computed by
\textsf{GeometricSolve} called with $\nV +
\binom{\nV+1}{n-d+1}\binom{n-i}{n-d+1} = O\!\left(\nV +
  \binom{\nV+1}{n-d+1}\binom{n}{n-d+1}\!\right)$ polynomials in $n$
variables. Each polynomial is given by a SLP of size
$\widetilde{O}\!\left(n^4\!\left(L+n^2\right)\right)$. Hence, the
input system is represented by a SLP of size $E$ in
$\widetilde{O}\left(\left(\nV +
    \binom{\nV+1}{n-d+1}\binom{n}{n-d+1}\!\right)
  n^4\!\left(L+n^2\right) \right)$. By Proposition
\ref{prop:degbounds}, $\delta\Par{\VVA{f^\bfA}{F^\bfA}{i}}$ is bounded
by
$D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$. Hence,
the computation can be done within
\[\widetilde{O}\left(s\Par{\nV+\binom{\nV+1}{n-d+1}\binom{n}{n-d+1}}
  LD^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)\]
arithmetic operations in $\Q$. Since $\binom{n}{n-d+1}\leq 2^n$, this
complexity is bounded by $\widetilde{O}\left(\left(s^2+s2^n\binom{\nV+1}{n-d+1}
  \right)LD^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$.

Likewise, $\crit{f^\bfA,\F^\bfA}$ is defined as the vanishing set of
\begin{itemize}
\item the polynomials $f^\bfA_1, \ldots, f^\bfA_\nV$,
\item the minors of size $n-d+1$ of $\jacc{\left[f^\bfA,\F^\bfA\right]}$.
\end{itemize}
Hence, the complexity of its computation by \textsf{GeometricSolve} is
the same as the above complexity of the computation of
$\VVA{f^\bfA}{F^\bfA}{i}$.

The computation of
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$
is done using \textsf{Difference}. Its complexity is in
$\widetilde{O}\left(ED^{3(n-d)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{(d+1)}\right)$.
%\left(\left(n-d+1\right)\left(D-1\right)\right)^{3n}\right)$.
It is dominated by the cost of the computation of
$\VVA{f^\bfA}{\F^\bfA}{i}$, thus we get the following complexity
result.
\begin{lemma}\label{lemma:complmodvp}
  There exists a probabilistic algorithm that takes as input
  $f^\bfA,\F^\bfA$ and $i$ and returns an equidimensional
  decomposition of
  $\ZariskiClosure{\VVA{f^\bfA}{F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$,
  encoded by a lifting fiber. In case of success,
  the algorithm has a complexity dominated by
  $\widetilde{O}\left(\left(s^2+s2^n\binom{\nV+1}{n-d+1}\right)
  LD^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$.
\end{lemma}


\subsubsection{Computation of $\VPC{f^\bfA}{\F^\bfA}{i}$}
Since $\VPC{f^\bfA}{\F^\bfA}{i}$ is defined as the intersection
$\displaystyle\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\critfVbfA}\cap\critfVbfA$,
a geometric resolution of each component of $\VPC{f^\bfA}{\F^\bfA}{i}$
is obtained from a set of irreducible lifting fibers of
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\critfVbfA}$. From
the output of the algorithm presented in Section \ref{sec:complexVVA},
a set of irreducible lifting fibers is recovered using
\textsf{SplitFiber} in time $\widetilde{O}\left(sE
  D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$. As
in Section \ref{sec:complexVVA}, the size $E$ is in
$\widetilde{O}\left(\left(\nV +
    \binom{\nV+1}{n-d+1}\binom{n}{n-d+1}\!\right)
  n^4\!\left(L+n^2\right) \right)$.
% The number of irreducible lifting fibers is at most
% $D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$.
The routine \textsf{LiftCurve} is used on each irreducible fiber in
order to obtain a parametrization of each component of the curve
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\critfVbfA}$. Lifting
one fiber is done in
\[\widetilde{O}\left(s\Par{\nV+\binom{\nV+1}{n-d+1}\binom{n}{n-d+1}}
  L D^{2(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{2(d+1)}\right).\]
% D^4\left(\left(n-d+1\right)\left(D-1\right)\right)^{2n}\right)

From such a parametrization, the routine
\textsf{OneDimensionalIntersect} is used with every polynomial that
defines $\critfVbfA$. There are $\binom{\nV+1}{n-d+1}\binom{n}{n-d+1}$
such polynomials, thus the cost to compute the rational
parametrization corresponding to one irreducible fiber is at
most \[\widetilde{O}\left(\binom{\nV+1}{n-d+1}\binom{n}{n-d+1} L
  D^{2(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{2(d+1)}\right).\]
The total cost for the
$D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$
irreducible lifting fibers is dominated by
$\widetilde{O}\left(s\Par{\nV+\binom{\nV+1}{n-d+1}\binom{n}{n-d+1}}
  LD^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$.
Finally, we compute a parametrization of the union of the zero-sets of
the previous parametrization using \cite[Lemma
9.1.3]{din2013nearly}. Since the sum of the degrees of each
parametrization is bounded by
$D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$, the
cost is negligible. Since $\binom{n}{n-d+1}\leq 2^n$, we get the
following result.

\begin{lemma}\label{lemma:complVPC}
  There exists a probabilistic algorithm that takes as input a set of
  lifting fibers of
  $\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\critfVbfA}$ and
  that returns a rational parametrization of
  $\VPC{f^\bfA}{\F^\bfA}{i}$. In case of success, the algorithm has a
  complexity dominated by
  $\widetilde{O}\left(\left(s^2+s2^n\binom{\nV+1}{n-d+1}\right)
    LD^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$.
\end{lemma}


\subsubsection{Complexity of \SetOfNonProperness{}}
As explained in \cite[Section 4]{Safey07}, the computation of the set of
non-properness of the restriction of the projection $\pi_T$ to
$\Variety{f^\bfA-T}\cap\left(\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}\times\C\right)$
from the representation of the variety
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$
can be done using a parametric geometric resolution
\cite{schost03}. Indeed, from a set of lifting fibers of
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$,
obtained by the routine \textsf{GeometricSolve}, one can compute a
geometric resolution of
$\Variety{f^\bfA-t}\cap\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$
for a generic $t\in\R$. Since there are at most
$D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}$ lifting
fibers, it is done using \textsf{OneDimensionalIntersect} on all the fibers
in $\widetilde{O}\Par{E
  D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}}$,
where as in Section \ref{sec:complexVVA}, $E$ is in
$\widetilde{O}\left(\left(\nV +
    \binom{\nV+1}{n-d+1}\binom{n}{n-d+1}\!\right) n^4\!\left(L+n^2\right)
\right)$.

From these geometric resolutions, \textsf{LiftParameter} computes a
parametric geometric resolution $(q,q_0,\dots,q_n)$ of
$\Variety{f^\bfA-T}\cap\left(\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}\times\C\right)$,
where $T$ is a parameter, in $\widetilde{O}\Par{E
  D^{3(n-d)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}}$.  As
explained in \cite[Section 4]{Safey07}, the set of non-properness is
contained in the roots of the least common multiple of the denominators of
the coefficients of the polynomial $q$. Since $\binom{n}{n-d+1}\leq 2^n$,
we get the following result.

\begin{lemma}\label{lemma:complSONP}
  There exists a probabilistic algorithm that takes as input a set of
  lifting fibers of
  $\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$
  and that returns a polynomial whose set of roots contains the set of
  non-properness of the projection $\pi_T$ restricted to
  $\Variety{f^\bfA-T}\cap\left(\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}\times\C\right)$. In
  case of success, the algorithm has a complexity dominated by
  $\widetilde{O}\Par{\left(s^2+s2^n\binom{\nV+1}{n-d+1}\right) L
    D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}}$.
\end{lemma}



\subsubsection{Complexity of \SamplePoints{} and \IsEmpty{}}
Given $\F=\left\{f_1,\dots,f_\nV\right\}$, an algorithm computing a
set of real sample points of $\Variety{\F}\cap\R^n$ is given in
\cite{SaSc}. It relies on the computation of polar varieties. Using
techniques described in \cite{BaGiHeMb01, BaGiHeMb97, din2013nearly}
and \cite[Section 3]{BGHSS}, a local description of the polar
varieties as a complete intersection can be obtained.  Assume that
$\Variety{\F}$ is equidimensional of dimension $d$. Such a local
description depends on the choice of a minor of size $n-d$ of the
Jacobian matrix $\jacc{\F}$. Since there are
$\binom{\nV}{n-d}\binom{n}{n-d}$ minors of size $n-d$ in $\jacc{\F}$,
a full description of the polar varieties is obtained by computing the
$\binom{\nV}{n-d}\binom{n}{n-d}$ possible localizations. Each local
description is given by a reduced regular sequence involving $n-d$
polynomials in $\F$ and minors of degree bounded by
$(n-d+1)(D-1)$. Hence, the routine \textsf{GeometricSolveRRS} computes
one local description in $\widetilde{O}\left(L
  D^{2(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{2(d+1)}
\right)$ so the cost for all localizations is in
$\widetilde{O}\left(\binom{\nV}{n-d}\binom{n}{n-d} L
  D^{2(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{2(d+1)}\right)$.
Note that in \cite{SaSc}, the complexity is cubic instead of quadratic
in the geometric degree of the inputs because these localization
techniques are not used to estimate the complexity.

Since
$\binom{n}{n-d}\leq 2^n$, this leads to the following complexity
result.
\begin{lemma}\label{lemma:complsample}
  There exists a probabilistic algorithm that takes as input $\F$
  satisfying assumptions $\assumptR$ and that returns a set of real
  sample points of $\Variety{F}\cap\R^n$, encoded by a rational
  parametrization. In case of success, the algorithm has a complexity
  dominated by $\widetilde{O}\left(2^n\binom{\nV}{n-d}L
    D^{2(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{2(d+1)}\right)$.
\end{lemma} 


\subsubsection{Complexity of \SetContaining{}}
The first step in \SetContaining{} is the computation of a set of real
sample points of $\Variety{\F^\bfA}\cap\R^n$. Its complexity is given
in Lemma \ref{lemma:complsample}. Then at the $i$-th step of the loop,
$\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}$,
the set of non-properness of the projection $\pi_T$ restricted to
$\Variety{f-T}\cap\left(\ZariskiClosure{\VVA{f^\bfA}{\F^\bfA}{i}\setminus\crit{f^\bfA,V^\bfA}}\times\C\right)$
and $\VPC{f^\bfA}{\F^\bfA}{i}$ are computed. The costs are given in
Lemma \ref{lemma:complmodvp}, Lemma \ref{lemma:complSONP} and Lemma
\ref{lemma:complVPC}. The complexity for one step is in
$\widetilde{O}\left(\left(s^2 + s2^n\binom{\nV+1}{n-d+1}\right)
  L D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$. Finally,
for the $d$ steps, since $d\leq n$ can be omitted, we get the
following complexity.

\begin{lemma}\label{lemma:complSC}
  In case of success, the routine \SetContaining{} performs at most
  $\widetilde{O}\left( \left(s^2 + s2^n \binom{\nV+1}{n-d+1}\right) L
    D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)$
  arithmetic operations in $\Q$.
\end{lemma}



\subsubsection{Complexity of \FindInfimum{}}
The most expensive steps in this routine are the calls to
\IsEmpty{}. There are at most $k$ such steps, where $k$ is the number
of points of non-properness, of critical values and of real sample
points. Using the Bézout inequality, $k$ lies in
$\widetilde{O}\Par{D^{n-d}\left(\left(n-d+1\right)\left(D-1\right)\right)^{d+1}}$. Using
the complexity estimate given in Lemma \ref{lemma:complsample}, this
leads to the following.

\begin{lemma}\label{lemma:complFI}
  In case of success, the routine \FindInfimum{} performs at most
  \[\widetilde{O}\left(2^n\binom{\nV}{n-d}L
    D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right).\]
\end{lemma}


\subsubsection{Complexity of the Algorithm}
Finally, the complexity of \Optimize{} comes from Lemma
\ref{lemma:complSC} and Lemma \ref{lemma:complFI}, using that
$\binom{s}{n-d}\leq \binom{s+1}{n-d+1}$.

\begin{theorem}\label{thm:complexity}
  In case of success, the algorithm \Optimize{} performs
\[\widetilde{O}\left(\left(s^2+s
  2^n \binom{\nV+1}{n-d+1}\right) L
  D^{3(n-d+1)}\left(\left(n-d+1\right)\left(D-1\right)\right)^{3(d+1)}\right)\]
arithmetic operations in $\Q$.
\end{theorem}

Remark that if $\F$ is a reduced regular sequence then the 
complexity is simpler.
\begin{theorem}
  If $\F$ is a reduced regular sequence, the algorithm \Optimize{}
  performs $\widetilde{O}\left(
    L\left(\sqrt[3]{2}\left(s+1\right)D\right)^{3(n+2)}\right)$
arithmetic operations in
  $\Q$.
\end{theorem}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "siopt_optimization_revision"
%%% End: 


==> implementation.tex <==
\section{Implementation and practical experiments}\label{sec:practical}
We give details about our implementation in Section
\ref{sec:implem}. Instead of using the geometric resolution algorithm
for algebraic elimination, we use Gr\"obner bases that still allow to
perform all geometric operations needed to implement the algorithm
(see \cite{cox} for an introduction to Gr\"obner bases). Moreover,
there exist practically efficient algorithms for computing Gr\"obner
bases \cite{F4, F5}.  This way, the probabilistic aspect of our
algorithm relies on the random choice of a linear change of
variables. In practice, we check whether the linear change of
variables is suitable. Thus one can guarantee exactness. This is
explained in Section \ref{sec:implem}.

In Sections \ref{sec:benchrandom} and \ref{sec:benchapplications}, we
present practical experiments. First, we run our implementation with
random dense polynomials, that is the hardest case for the inputs.  As
an example, our implementation can solve problems with an objective
polynomial and one constraint, both of degree $2$, with up to $32$
variables using $4$ hours of CPU time. With two constraints, our
implementation can solve problems with up to $11$ variables using
$5.3$ hours of CPU time. With a linear objective polynomial subject to
one constraint of degree $4$, both in $5$ variables, it takes $34$
minutes. These results show that our implementation outperforms
general symbolic solvers based on the Cylindrical Algebraic
Decomposition.

Then we run examples coming from applications. Some of these examples
can be solved by QEPCAD. The timings are given in Section
\ref{sec:benchapplications}.

% Thanks to a private communication with D. Henrion, it appears that
% tools based on moment relaxations like GloptiPoly \cite{GloptiPoly}
% are designed to solve global optimization problems on bounded sets or
% for which the infimum is reached. These assumptions are either
% difficult to check automatically or not satisfied for most of our
% examples, hence it is meaningless to compare our implementation with
% such tools. Likewise, w
We do not report timings of methods based on sums of squares or
numerical procedures, e.g. \cite{YALMIP, SOSTOOLS, GloptiPoly} since
their outputs are numerical approximation while our algorithm provides
exact outputs.

\subsection{Implementation}\label{sec:implem}
Since our algorithm depends on the choice of a matrix that defines a
change of coordinates, it is probabilistic. However, we present a
technique to make sure that this choice is a correct one. This
technique is used in our implementation.

As stated in Section \ref{sec:correctness}, the algorithm is correct
if the subroutines \SetContaining{} and \FindInfimum{} are
correct. According to Proposition \ref{prop:SetContainingcorrect}, if
the random matrix chosen at the first step of \Optimize{} is such that
$\PropPJSC{f^\bfA,\F^\bfA}$, $\PropPISSAC{f^\bfA,\F^\bfA}$ and
$\PropReg{f^\bfA,\F^\bfA}$ hold, then \SetContaining{} runs
correctly. Then its output satisfies property $\PropOpt{W(f, \F),
  V(\F)}$. Hence, \FindInfimum{} can be called with the output of
\SetContaining{}.

Then the choice of the matrix $\bfA$ leads to a correct output if
$\PropPJSC{f^\bfA,\F^\bfA}$, $\PropPISSAC{f^\bfA,\F^\bfA}$ and
$\PropReg{f^\bfA,\F^\bfA}$ hold.

Property $\PropReg{f,\F}$ always holds if $\F$ satisfies assumptions
$\assumptR$ (see \cite[Lemma 2.2]{GrGuSaZh}). Since for any change of
coordinates, $\F$ satisfies assumptions $\assumptR$ if and only if
$\F^\bfA$ does, $\PropReg{f^\bfA,\F^\bfA}$ holds for any
$\bfA\in\GLnQ$. Then it remains to check $\PropPJSC{f^\bfA,\F^\bfA}$
and $\PropPISSAC{f^\bfA,\F^\bfA}$. Both properties depend on the
properness of projections of the form
\[\fonction{\ProjLeft{d}}{W\subset\C^n}{\C^d}{(x_1, \ldots, x_n)}{\left(x_1,\dots, x_d\right)}\]
where $W$ is an algebraic variety. According to \cite[Proposition
3.2]{jelonek}, if $I_V$ is an ideal such that $V=\Variety{I_V}$ has
dimension $d$ then the projection
\[\fonction{\ProjLeft{d}}{V\subset\C^n}{\C^d}{(x_1, \ldots, x_n)}{\left(x_1,\dots, x_d\right)}\]
is proper if and only if $I_V$ is in Noether position.

Thus we choose the matrix $\bfA$ such that after the change of
variables, the ideals are in Noether position. This can be done using
techniques described in \cite[Section 4.1.2]{KrPaSo01} and
\cite{logar89}. These techniques are used in our implementation to
obtain a matrix as sparse as possible that makes \SetContaining{}
correct.



\subsection{Practical experiments}\label{sec:benchrandom}
The analysis of the degree of the algebraic varieties involved in the
computations provides a singly exponential bound in the number of
indeterminates. This matches the best complexity bounds for global
optimization algorithms using quantifier elimination.  Our
implementation is written in Maple. Gr\"obner bases are computed using
the package FGb \cite{fgb} (\url{http://www-polsys.lip6.fr/~jcf/Software/}.)

The computations were performed on a Intel Xeon CPU E7540 @ 2.00GHz
and 250GB of RAM.

In the tables below, we use the following notations:
\begin{itemize}
\item $d$: degree of the objective polynomial $f$;
\item $D$: upper bound for the degree of the constraints;
\item $n$: number of indeterminates;
\item $\nV$: number of constraints;
\item obj terms: number of terms in the objective polynomial;
\item terms: average number of terms.
\end{itemize}

To test the behavior of the algorithm, we run it with randomly
generated polynomials and constraints as inputs.

Considering an objective polynomial and one constraint, both of degree
$2$ and increasing the number of variables, our implementation can
solve problems with up to $32$ variables in $4$ hours. For this
special case, the algorithm seems to be sub-exponential.

\paragraph{Constraints of degree 2}~
{\small\begin{center}
  \begin{tabular}{|ccccccc|}\hline
    \input{Maple/tests/results_densedegree2.txt}
    \hline
  \end{tabular}
\end{center}}

% In the following, it can be seen that the practical results match the
% single exponential complexity.

\paragraph{Constraints of degree 3}~
{\small \begin{center}
  \begin{tabular}{|ccccccc|}\hline
    \input{Maple/tests/results_densedegree3.txt}
    \hline
  \end{tabular}
\end{center}}


\paragraph{Constraints of degree 4}~
{\small \begin{center}
  \begin{tabular}{|ccccccc|}\hline
    \input{Maple/tests/results_densedegree4.txt}
    \hline
  \end{tabular}
\end{center}}

\paragraph{Linear objective function}~
{\small \begin{center}
  \begin{tabular}{|ccccccc|}\hline
    \input{Maple/tests/results_denselinearobj.txt}
    \hline
  \end{tabular}
\end{center}}


\subsection{Examples coming from applications}\label{sec:benchapplications}
We consider examples coming from applications to compare the execution
time of our algorithm with a cylindrical algebraic decomposition
algorithm. These decompositions are computed using QEPCAD version B
1.69\footnote{Implementation originally due to H. Hong, and
  subsequently added on to by C. W. Brown, G. E. Collins,
  M. J. Encarnacion, J. R. Johnson, W. Krandick, S. McCallum,
  S. Steinberg, R. Liska, N. Robidoux. Latest version is available at
  \url{http://www.usna.edu/cs/~qepcad/}.} These examples are described
in Appendix \ref{appendix:examples} and available as a plain text file
openable with Maple at \url{http://www-polsys.lip6.fr/~greuet/}.

{\small\begin{center}
  \begin{tabular}{|ccccccccc|} \hline
    \input{Maple/tests/results_exemples_qepcad.txt}
    \hline
  \end{tabular}
\end{center}}

\appendix
\section{Description of examples}\label{appendix:examples}
\begin{example}{nonreached, nonreached2}
  Let $g\left(x_1,x_2,x_3\right) = x_1^2-x_1x_2+x_1x_2x_3+x_2+3$ and
  consider the two problems
  \[\left\{\begin{array}{rl}
    \inf_{x\in \mathbb{R}^3} & (x_1x_2-1)^2+x_2^2 + x_3^2 + 42\\
    \text{s.t. } & \ x_3 = 0. \\
  \end{array}\right.\]
 \[\left\{\begin{array}{rl}
    \inf_{x\in \mathbb{R}^3} & (x_1x_2-1)^2+x_2^2 + x_3^2g + \left(x_1+1\right)g^3 + 42\\
    \text{s.t. } & \ g\left(x_1,x_2,x_3\right) = 0. \\
  \end{array}\right.\]
Their infima are not reached. They are the limit of sequences
$f(z_k)$, where $\left\|z_k\right\|$ tends to infinity. For instance,
$z_k$ can be of the form $\left(x^{(k)}_1,\frac{1}{x^{(k)}_1},x^{(k)}_3\right)$, where
$x^{(k)}_1$ tends to infinity. Note that both examples cause instabilities
to numerical algorithms.
\end{example}


\begin{example}{isolated}
  It is a toy example: $f^\star$ is isolated in $f\left(V\cap\R^n\right)$.
  \[\left\{\begin{array}{rl}
    \inf_{x\in \mathbb{R}^2} & \left(x_1^2+x_2^2-2\right)\left(x_1^2+x_2^2\right)\\
    \text{s.t. } & \ \left(x_1^2+x_2^2-1\right)\left(x_1-3\right) = 0. \\
  \end{array}\right.\]
On $V\cap\R^n$, either $x_1^2+x_2^2 = 1$ or $x_1 = 3$. Then the
objective polynomial is either equal to $-1$ or
$\left(7+x_2^2\right)\left(9+x_2^2\right)$. The second expression is
positive over the reals.
\end{example}


\begin{example}{reachedasympt}
  The infimum is both attained and an asymptotic value. Indeed,
  $f^\star = 42$ is reached at any point $\left(x_1,0,0\right)$, but
  is also the limit of sequences of the form
  $\left(x_1,\frac{1}{x_1},0\right)$ when $x_1$ tends to
  infinity. Some iterative methods do not return a minimizer close to
  $\left(x_1,0,0\right)$.
  \[\left\{\begin{array}{rl}
    \inf_{x\in \mathbb{R}^3} & \left(10000\left(x_1x_2-1\right)^4 + x_1^6\right)x_2^6 + \frac{1}{124}x_3^2 + 42\\
    \text{s.t. } & \ x_3 = 0. \\
  \end{array}\right.\]
\end{example}

\begin{example}{GGSZ2012}%jsc44.mpl
  It comes from \cite{GrGuSaZh} (Example 4.4). The minimizer does not
  satisfy the KKT conditions.
  \[\left\{\begin{array}{rl}
      \inf_{x\in \mathbb{R}^2} & (x_1+1)^2+x_2^2\\
      \text{s.t. } & \ x_1^3 = x_2^2. \\
  \end{array}\right.\]
\end{example}



\begin{example}{Nie2011}%Nie2010.mpl
  It comes from \cite{NieExact2011} (Example 5.2). It has been studied
  in \cite{GrGuSaZh} because of the numerical instabilities that
  occurs with numerical algorithms.
  \[\left\{\begin{array}{rl}
  \inf_{x\in \mathbb{R}^3} & x_1^6+x_2^6+x_3^6+3x_1^2x_2^2x_3^2-x_1^2(x_2^4+x_3^4)-x_2^2(x_3^4+x_1^4)-x_3^2(x_1^4+x_2^4)\\
  \text{s.t. } & \ x_1+x_2+x_3-1 = 0. \\
  \end{array}\right.\]
\end{example}



\begin{example}{LaxLax}%laxlax
  The objective polynomial appears in \cite{laxlax} and
  \cite{KLYZ12}. Its infimum is $0$ and is reached over $V\left(x_1 ,
    x_2 - x_3, x_3 - x_4\right)\cap\R^n$.
  \[\left\{\begin{array}{rl}
      \inf_{\left(x\right)\in \mathbb{R}^4} & x_1x_2x_3x_4 - x_1\left(x_2 - x_1\right)\left(x_3 - x_1\right)\left(x_4 - x_1\right)\\
      & - x_2\left(x_1 - x_2\right)\left(x_3 - x_2\right)\left(x_4 - x_2\right) - x_3\left(x_1 - x_3\left)\right
        (x_2 - x_3\right)\left(x_4 - x_3\right)\\
      & - x_4\left(x_1 - x_4\right)\left(x_2 - x_4\right)\left(x_3 - x_4\right)\\
      \text{s.t. } & x_1 =  x_2 - x_3 =  x_3 - x_4 = 0.
  \end{array}\right.\]
\end{example}



\begin{example}{maxcut5-1/5-2}%maxcut5-1
  A cut of a graph with weighted edges is a partition of the vertices
  into two disjoint subsets. Its weight is the sum of the weights of
  the edges crossing the cut. The maxcut problem is to find a cut
  whose weight is greater than or equal to any other cut.  This
  problem has applications, among other, in very-arge-scale
  integration circuit design and statistical physics \cite{DeLa,
    FePaReRi}. It can be reformulated has a constrained polynomial
  optimization problem \cite{commander}. For a graph of $p$ vertices
  and weight $w_{ij}$ for the edge joining the $i$-th vertex to the
  $j$-th one, it is equivalent to solve
  \[\left\{\begin{array}{rl}
      \inf_{x\in \mathbb{R}^p} & \,\,\,\, - \frac{1}{2}\sum_{1\leq i < j \leq p} w_{ij}\left( 1 - x_ix_j\right)\\
      \text{s.t. } & x_i^2 - 1 = 0, \text{ for } i\in\left\{1,\dots, p\right\}, \\
    \end{array}\right.\]
  We use the set of weight $W_{G5-1}$ and $W_{G5-2}$ in \cite{BaBu},
  that leads to solve
  \[\left\{\begin{array}{rl}
      \inf_{x\in \mathbb{R}^5} & -98 + \frac{23}{2} x_1x_2 + 8 x_1x_3 + 9 x_1x_4 + \frac{17}{2}x_1x_5 + \frac{25}{2} x_2x_3 \\
      &  + 13 x_2 x_4 +\frac{23}{2} x_2 x_5 + 7x_3x_4 + 12 x_3x_5 + 5x_4x_5\\
      \text{s.t. } & x_i^2 - 1 = 0, \text{ for } i\in\left\{1,\dots, 5\right\}.\\
    \end{array}\right.\]
  and
  \[\left\{\begin{array}{rl}
    \inf_{x\in \mathbb{R}^5} &-31+3x_1x_2+3x_1x_3+4x_1x_4+5x_1y_5+\frac52x_2x_3+\frac52x_2x_4+3x_2x_5\\
    & +2x_3 x_4+3x_3x_5+3x_4x_5\\
    \text{s.t. } & x_i^2 - 1 = 0, \text{ for } i\in\left\{1,\dots, 5\right\}.\\
  \end{array}\right.\]
\end{example}




\begin{example}{coleman5/6}%coleman5/coleman6
  They come from optimal control problems and appears in
  \cite{coleman}.  For $M\in\left\{5,6\right\}$, let
  $x_1,\dots,x_{M-1}$ and $y_1,\dots,y_{M-1}$ be the indeterminates.
  \[\left\{\begin{array}{rl}
      \inf_{\left(x,y\right)\in \mathbb{R}^{2M}} & \,\,\,\, 
      \frac{1}{M}\sum_{i = 1}^{M-1} x_i^2 + y_i^2\\
      \text{s.t. } & y_1 - 1 =  y_{i+1} - y_i - \frac{1}{M-1}\left(y_i^2 - x_i\right) = 0, \text{ for } i\in\left\{1,\dots, M-2\right\}.
  \end{array}\right.\]
\end{example}



\begin{example}{Vor1}
  It comes from \cite{Vor} and have no constraints. It is too large to
  be written here but can be found at
  \url{http://www-polsys.lip6.fr/~greuet/}.
\end{example}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "siopt_optimization_revision"
%%% End: 

==> intro.tex <==
\section{Introduction}

Let $\bfX=X_1, \ldots, X_n$ be indeterminates, $f, f_1, \ldots, f_\nV$
be polynomials in $\PolRing$ of maximal degree $D$ and $V=V(\F)$ be
the set of common complex solutions of $\F=(f_1,\ldots, f_\nV)$. We
focus on the design and the implementation of {\em exact} algorithms
for solving the polynomial optimization problem which consists in
computing and exact representation of the global infimum
$f^\star=\inf_{x\in V\cap\R^n} f\left(x\right)$.  It is worth to note
that, at least under some genericity assumptions, polynomial
optimization problems whose constraints are non-strict inequalities
can be reduced to the one with polynomial equations (see
e.g. \cite{BGHS14} and references therein).



% Let $\bfX=\Par{X_1,\dots,X_n}$, $\F =
% \left\{f_1,\dots,f_\nV\right\}\subset\PolRing$ and $V\subset \C^n$ be
% the algebraic variety $\Variety{\F} = \left\{x\in\C^n\mid
%   f_1\Par{x}=\cdots=f_\nV\Par{x}=0\right\}$. Given another polynomial
% $f\in\Q\left[\bfX\right]$, we consider the global polynomial
% optimization problem: compute the global infimum $f^\star=\inf_{x\in
%   V\cap\R^n} f\left(x\right)$. 
% Note that, at least under some
% genericity assumptions, polynomial optimization problems whose
% constraints are non-strict inequalities can be reduced to the one with
% polynomial equations.

\paragraph*{Motivation and prior work}
While polynomial optimization is well-known to be {\cal NP}-hard (see
e.g. \cite{nesterov00}), it has attracted a lot of attention since it
appears in various areas of engineering sciences (e.g. control theory
\cite{PositivePolControl,HSK03}, static analysis of programs
\cite{Cousot05,Monniaux10}, computer vision \cite{AhAgTh12, AhStTh11},
economics, etc.). In this area, one challenge is to
combine practical efficiency with reliability for polynomial
optimization solvers.

One way to reach this goal is to relax the polynomial optimization
problem by computing algebraic certificates of positivity proving
lower bounds on $f^\star$. This is achieved with methods computing
sums of squares decompositions of polynomials. In this context, one
difficulty is to overcome the fact that a nonnegative polynomial is
not necessarily a sum of squares. Various techniques have been
studied, see e.g. \cite{DeNiPo07, GrGuSaZh, Vui-constraints,
  GloptiPoly, lasserre01globaloptimization, NiDeSt,
  schweighofer}. These approaches use semi-definite programming
relaxations (\cite{parriloPHD, shor}) and numerical solvers of
semi-definite programs.  Sometimes, a sum of squares decomposition
with rational coefficients can be recovered from such a decomposition
computed with floating point coefficients (see \cite{KLYZ12, PaPe}).
Algorithms for computing sums of squares decompositions with rational
coefficients have also been designed \cite{QSZ13, SZ10}. Some cases of
ill-conditionedness have been identified (\cite{gcv_sos}), but there
is no general method to overcome them. It should also be noticed that
techniques introduced to overcome situations where a non-negative
polynomial is not a sum of squares rely on using gradient varieties
\cite{DeNiPo07, GrGuSaZh, NiDeSt} which are close to polar varieties
introduced in the context of symbolic computation for studying real
algebraic sets (see e.g. \cite{BaGiHeMb97, BaGiHeMb01, BGHSS, SaSc}),
quantifier elimination (see e.g. \cite{HS09, HS12}) or connectivity
queries (see e.g. \cite{SaSc11, din2013nearly}).

% However, reliable algorithms are needed, for instance in program
% verification. Symbolic algorithms can provide this kind of reliable
% algorithm, but the complexity has to be managed.

Another way to combine reliability and practical efficiency is to
design algorithms relying on symbolic computation that solve the
polynomial optimization problem. Indeed, it can be seen as a special
quantifier elimination problem over the reals and a goal would be to
design a dedicated algorithm whose complexity meets the best known
bounds and whose practical behaviour reflects its complexity. 


Quantifier elimination over the reals can be solved by the cylindrical
algebraic decomposition algorithm \cite{Collins75}. This algorithm
deals with general instances and has been studied and improved in many
ways (see e.g. \cite{Brown99, Collins98, CollinsHong, Hong92,
  McCallum98}). However, its complexity is doubly exponential in the
number of variables. In practice, its best implementations are limited
to non trivial problems involving $4$ variables at most.

In \cite{BPR96}, a deterministic algorithm whose complexity is singly
exponential in the number of alternations of quantifiers is given. On
polynomial optimization problems, this specializes to an algorithm for
polynomial optimization that runs in time $D^{O(n)}$ (see
\cite[Chapter 14]{BaPoRo06}). The techniques used to get such
complexity results such as infinitesimal deformations did not provide
yet practical results that reflect this complexity gain. While in some
special cases, practical algorithms for one-block quantifier
elimination problems have been derived by avoiding the use of
infinitesimals \cite{HS09, HS12}, the problem of obtaining fast
algorithms in theory and in practice for polynomial optimization
remained open.

Thus, our goal is to obtain an efficient algorithm for solving the
polynomial optimization problem in theory and in practice. Thus, we
expect its complexity to lie within $D^{O(n)}$ operations but with a
good control on the complexity constant in the exponent. We allow to
have regularity assumptions on the input that are reasonable in
practice (e.g. rank conditions on the Jacobian matrix of the input
equality constraints). We also allow probabilistic algorithms provided
that probabilistic aspects do not depend on the input but on random
choices performed when running the algorithm.

% The use of algebraic techniques to solve optimization problem implies the manipulation of objects whose degree is
% intrinsically higher than the input.

% The use of algebraic techniques increases the degree of the considered
% objects \cite{JePeTs}. A fundamental problem is then to get both
% theoretical and practical efficiency, even by considering
% probabilistic algorithms. To this end, the constant factor in the
% exponent must be well controlled.

A first attempt towards this goal is in \cite{Safey08}. Given a
$n$-variate polynomial $f$ of degree $D$, a probabilistic algorithm
computing $\displaystyle\inf_{x\in\R^n}f\Par{x}$ in $\bigO{n^7D^{4n}}$
operations in $\Q$ is given. Moreover, it is practically efficient
and has solved problems intractable before (up to $6$ variables). Our
goal is to generalize this approach to the case of equality
constraints and get an algorithm whose complexity is essentially cubic
in $\Par{\nV D}^n$ and linear in the evaluation complexity of the input. 


\paragraph*{Main results} We provide a probabilistic algorithm based
on symbolic computation solving the polynomial optimization problem up
to some regularity assumptions on the equality constraints whose
complexity is essentially cubic in $\Par{\nV D}^n$. We also provide an
implementation of it and report on its practical behaviour which
reflects its complexity and allows to solve problems that are either
hard from the numerical point of view or unreachable by previous
algorithms based on symbolic computation.


Before describing these contributions in detail, we start by stating
our regularity assumptions which hold on the equality constraints. In
most of applications, the Jacobian matrix of $\F=(f_1, \ldots, f_\nV)$
has maximal rank at all points of the set of common solutions of
$\F$. In algebraic terms, this implies that this solution set is
smooth of co-dimension $\nV$, complete intersection and the ideal
generated by $\F$ (i.e. the set of algebraic relations generated by
$\F$) is radical.

Our regularity assumptions are a bit more general than the situation
we just described. In the sequel, we say that $\F$ satisfies 
assumption $\assumptR$ if the following holds:
% Recall that the considered problem is the computation, given
% $f\in\PolRing$ and $\F=\left\{f_1,\dots,f_\nV\right\}\subset\PolRing$,
% of $f^\star = \inf_{x\in\Variety{\F}\cap\R^n}f\Par{x}$. We provide a
% symbolic algorithm solving this problem under the following
% assumptions $\assumptR$:
\begin{itemize}
\item the ideal $\IdealAngle{\F}$ is radical,
\item $\Variety{\F}$ is equidimensional of dimension $d>0$,
\item $\Variety{\F}$ has finitely many singular points.
\end{itemize}

% These assumptions are far for being restrictive since they often hold
% in practice. For instance, any set of polynomials
% $\F=\left\{f_1,\dots,f_\nV\right\}\subset\PolRing$ that generate a
% radical ideal of dimension $n-s$ and whose Jacobian matrix has full
% rank satisfies them.
Under these assumptions, we provide an algorithm that decides the
existence of $f^\star= \inf_{x\in\Variety{\F}\cap\R^n}f\Par{x}$ and,
whenever $f^\star$ exists, it computes an exact representation of it (i.e. a
univariate polynomial vanishing at $f^\star$ and an isolating interval
for $f^\star$).  It can also decide if $f^\star$ is reached and if
this is the case it can return a minimizer $x^\star$ such that
$f\Par{x^\star}=f^\star$. 

We count arithmetic operations $+, -, \times, \div$ in $\Q$ and sign
evaluation at unit cost. We use the soft-O notation:
$\widetilde{O}(a)$ indicates the omission of polylogarithmic factors
in $a$.  The complexity of the algorithm described in this paper is
essentially cubic in $\Par{\nV D}^n$ and linear in the complexity of
evaluating $f$ and $\F$. For instance if the Jacobian matrix of $\F$
has full rank at all points of $\Variety{\F}$ (this is a bit more
restrictive than $\assumptR$) then the algorithm performs
\[\widetilde{O}\left(
    L\left(\sqrt[3]{2} \left(s+1\right)D\right)^{3(n+2)}\right)\]
arithmetic operations in $\Q$ (see Theorem \ref{thm:complexity} for
the general case in Section \ref{sec:complexity}).

% The algorithm works if some technical properties of genericity are
% satisfied. To ensure these properties, a generic change of coordinates
% is performed, making the algorithm probabilistic. However, we show how
% to test whether the genericity properties hold, so that we can be sure
% that the algorithm return the right answer.

% It has been implemented in Maple. With our implementation, we are able
% to solve problems unreachable with the previous symbolic
% methods. Furthermore, problems that seems difficult with numerical
% approaches are solved efficiently too.

% To illustrate its theoretical efficiency, we state the main result in
% a simpler case. See also Section \ref{sec:complexity} for a complexity
% estimate in the general case. The $\widetilde{O}$ notation means that
% we omit the logarithmic factors.

% \begin{theorem}
%   Let $f_1, \ldots, f_s$ and $f$ be polynomials with rational
%   coefficients in the indeterminates $X_1, \ldots, X_n$ of degree
%   bounded by $D$ be given by a straight-line program of length
%   $L$. Assume that $\F=(f_1, \ldots, f_s)$ satisfies $\assumptR$.
%   There exists a probabilistic algorithm which takes as input $\F$ and
%   $f$


  % input
  % \begin{itemize}
  % \item $\F=\left\{f_1,\dots,f_\nV\right\}\subset\PolRing$ that generates a radical ideal of dimension $n-s$ such that the
  %   Jacobian matrix associated with $f_1,\dots,f_\nV$ has rank $s$,
  % \item $f\in\PolRing$,
  % \end{itemize}
  % and that

%   and returns an exact representation of $\displaystyle f^\star =
%   \inf_{x\in\Variety{\F}\cap\R^n}f\Par{x}$. If $f^\star$ is reached,
%   it also returns $x^\star\in\Variety{\F}\cap\R^n$ such that
%   $f\Par{x^\star}=f^\star$. This algorithm requires at most 
%   \[\widetilde{O}\left(\left(L+n^2\right)
%     D^3\left(\sqrt[3]{2}\left(s+1\right)\left(D-1\right)\right)^{3n}\right)\]
%   arithmetic operations in $\Q$.
% \end{theorem}

Note that this algorithm is a strict generalization of the one given
in \cite{Safey08}. Note also that when the infimum is reached, we
compute a minimizer without any assumption on the dimension of the set
of minimizers.

Our algorithm follows a classical pattern which is used for quantifier
elimination over the reals. It first performs a change of coordinates
to ensure some technical assumptions that are satisfied in general
position. Then, roughly speaking, it computes an ordered finite set of
real numbers containing $f^\star$. Moreover, for any interval between
two consecutive numbers in this set is either contained in
$f\left(\Variety{\F}\cap\R^n\right)$ or has an empty intersection with
$f\left(\Variety{\F}\cap\R^n\right)$.

To compute this set, we use geometric objects which are close to the
notion of polar varieties which, under $\assumptR$, are critical loci
of some projections ; we refer to \cite{BGHSS} for more details on 
several properties of polar varieties and to \cite{BGHS14} for
geometric objects similar to the ones we manipulate in a more
restrictive context. Our modified polar varieties are defined
incrementally and have a degree which is well controlled (essentially
singly exponential in $n$). Algebraic representations of these
modified polar varieties can be computed using many algebraic
algorithms for polynomial system solving. Properties of the systems
defining these modified polar varieties are exploited by some
probabilistic algebraic elimination algorithms (see e.g. the geometric
resolution algorithm \cite{GiLeSa01} and references therein) which
allows to state our complexity results.


Our implementation is based on Gr\"obner basis computations which have
a good behaviour in practice (see also \cite{FGS13, Sp13} for
preliminary complexity estimates explaining this behaviour). Recall
that most of algorithms for computing Gr\"obner bases are
deterministic.  This implementation is available at
\url{http://www-polsys.lip6.fr/~greuet/}. We describe it in Section
\ref{sec:practical}; in particular, we show how to check if the
generic assumptions required for the correctness are satisfied after
performing a linear change of coordinates.  We report on experiments
showing that its practical performances outperform other
implementations of previous algorithms using symbolic computation and
can handle non-trivial problems which are difficult from the numerical
point of view.

% After the change of variables, there are two main steps in the
% algorithm. First, a finite subset of $\R$ containing all the local
% extrema is computed. It is done by computing values that satisfy a
% necessary condition to be an extremum. This condition is stated and
% proved in the paper. Finally, one wants to decide which value in the
% previous set is actually $f^\star$. To this end, we use a topological
% property provided in this paper. It reduces the problem to test the
% emptiness of finitely many real fibers of $f$.




\paragraph*{Plan of the paper}
We introduce notations and definitions of geometric objects in Section
\ref{sec:notations}. Section \ref{sec:algo} describes the algorithm
and its subroutines. Section \ref{sec:correctness} is devoted to the
proof of correctness of the algorithm, under some geometric
assumptions on some geometric objects depending on the input. Then in
Section \ref{sec:generic}, we prove that these assumptions are true up
to a generic change of coordinates on the input. Finally, the
complexity is analyzed in Section \ref{sec:complexity}. Some details
on the implementation and practical results are presented in Section
\ref{sec:practical}.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "siopt_optimization_revision"
%%% End: 

